TOI-2076 and TOI-1807: Two young, comoving planetary systems within 50 pc identified by TESS that are ideal candidates for further follow-up

We report the discovery of two planetary systems around comoving stars; TOI-2076 (TIC 27491137) and TOI-1807 (TIC 180695581). TOI-2076 is a nearby (41.9 pc) multi-planetary system orbiting a young (204$\pm$50 Myr), bright (K = 7.115 in TIC v8.1). TOI-1807 hosts a single transiting planet, and is similarly nearby (42.58pc), similarly young (180$\pm$40 Myr), and bright. Both targets exhibit significant, periodic variability due to star spots, characteristic of their young ages. Using photometric data collected by TESS we identify three transiting planets around TOI-2076 with radii of R$_b$=3.3$\pm$0.04$R_\oplus$, R$_c$=4.4$\pm$0.05$R_\oplus$, and R$_d$=4.1$\pm$0.07$R_\oplus$. Planet TOI-2076b has a period of P$_b$=10.356 d. For both TOI 2076c and d, TESS observed only two transits, separated by a 2-year interval in which no data were collected, preventing a unique period determination. A range of long periods (>17d) are consistent with the data. We identify a short-period planet around TOI-1807 with a radius of R$_b$=1.8$\pm$0.04$R_\oplus$ and a period of P$_b$=0.549 d. Their close proximity, and bright, cool host stars, and young ages, make these planets excellent candidates for follow-up. TOI-1807b is one of the best known small ($R<2R_\oplus$) planets for characterization via eclipse spectroscopy and phase curves with JWST. TOI-1807b is the youngest ultra-short period planet discovered to date, providing valuable constraints on formation time-scales of short period planets. Given the rarity of young planets, particularly in multiple planet systems, these planets present an unprecedented opportunity to study and compare exoplanet formation, and young planet atmospheres, at a crucial transition age for formation theory.

==> GJ1214_comp.tex <==

\begin{table}
\centering
\caption{\scriptsize{Best known planets $<4.5R_\Earth$ for transmission spectroscopy}}
\begin{threeparttable}
\begin{tabular}{@{}lclc@{}}
\toprule
Planet name & \multicolumn{1}{l}{$R_p/(R_\Earth$)} & S/N$^a$   & Source \\ \midrule
GJ 1214 b   & $2.847^{+0.202}_{-0.202}$            & 1.000 & \cite{GJ1214b} \\
\textbf{TOI-2076 c}  & $4.471^{+0.044}_{-0.048}$   & \textbf{0.799} & This work\\
\textbf{TOI-2076 d}  & $3.888^{+0.068}_{-0.068}$   & \textbf{0.780} & This work \\
Pi Men c             & $2.042^{+0.05}_{-0.05}$     & 0.612 & \cite{PiMenC_R}          \\
LTT 1445 A b         & $1.38^{+0.13}_{-0.13}$      & 0.572 & \cite{LTT1445}           \\
55 Cnc e             & $1.91^{+0.08}_{-0.08}$      & 0.533 & \cite{55Cnc}           \\
\textbf{\textbf{TOI-2076 b}}  &$3.384^{+0.044}_{-0.045}$ & \textbf{0.533} & This work \\
HAT-P-11 b             & $4.36^{+0.06}_{-0.06}$     & 0.504 & \cite{HAT}          \\
HD 63433 c           & $2.67^{+0.12}_{-0.12}$      & 0.495 & \cite{HD63433}           \\
HD 63433 b           & $2.15^{+0.10}_{-0.10}$      & 0.472 & \cite{HD63433}           \\
HD 219134 b          & $1.602^{+0.055}_{-0.055}$   & 0.461 & \cite{HD219134} \\
\hspace{7mm} \vdots & \vdots & \hspace{3.5mm}\vdots & \vdots  \\
\textbf{\textbf{TOI-1807 b$^*$}}  &$1.526^{+0.944}_{-0.944}$ & \textbf{0.064} & \textcolor{red}{cite}\\\bottomrule
\end{tabular}
        \begin{tablenotes}
            \item[a] Following the process implemented in table 3 of \cite{superE}, S/N values are relative to GJ 1214 b.
            \item[*] TOI-1807 b has been included for completeness. It is actually the \textcolor{red}{X} most amenable planet for transmission spectroscopy. 
        \end{tablenotes}
        \end{threeparttable}
\label{tab: obs_comp}
\end{table}



==> authors.tex <==
\correspondingauthor{Christina Hedges}
\email{christina.l.hedges@nasa.gov}
\author{Christina Hedges}
\affiliation{\BayArea}
\affiliation{\ames}

% CONFIRMED
% UG Student, identified transits by eye
\author{Alex Hughes}
\affiliation{Department of Physics, Loughborough University, Epinal way, Loughborough, Leicestershire, LE11 3TU, UK}

% Confirmed
% Age calculations
\author[0000-0002-4891-3517]{George Zhou}
\affiliation{\usq}


% Young star discussion
\author[0000-0001-6534-6246]{Trevor J.\ David}
\affiliation{\flatiron}

% Period aliasing 
\author[0000-0002-7733-4522]{Juliette Becker}
\affiliation{\DGPScaltech}


% Confirmed
% False positive probability, student studying with Courtney
\author[0000-0002-8965-3969]{Steven Giacalone}
\affil{\berkely}



% Vetting, All round heavy hitter
\author[0000-0001-7246-5438]{Andrew Vanderburg}
\affiliation{\wisconsin}

% I think confirmed
% SED Fitting
\author[0000-0001-8812-0565]{Joseph E. Rodriguez} 
\affiliation{\msu}

% Stellar parameter fitting
\author[0000-0001-6637-5401]{Allyson Bieryla} 
\affiliation{\cfa}


%confirmed
% Student with George working on Lithium Abundances
\author{Christopher Wirth}
\affiliation{Harvard University, Cambridge, MA 02138, USA.}
\affiliation{\cfa}


% CONFIRMED
% Supervisor and mentor for Alex
\author[0000-0002-6544-1523]{Shaun Atherton}
\affiliation{Department of Physics, Loughborough University, Epinal Way, Loughborough, Leicestershire, UK, LE11 3TU}


% Confirmed
% Looked into phase curves
\author[0000-0002-3551-279X]{Tara Fetherolf}
\affiliation{\riverside}

%Confirmed?
%karen.collins@cfa.harvard.edu  (TFOP SG1 organization, LCO scheduling and data reduction)
\author[0000-0001-6588-9574]{Karen A.\ Collins}
\affiliation{\cfa}


% CONFIRMED
% Gaia discussion
\author[0000-0001-6534-6246]{Adrian M. Price-Whelan}
\affiliation{\flatiron}

%confirmed
% Radial velocity discussion
\author[0000-0001-9907-7742]{Megan Bedell}
\affiliation{\flatiron}

% confirmed
\author[0000-0002-8964-8377]{Samuel N. Quinn} 
\affiliation{\cfa}

% confirmed
%tjgan@foxmail.com (LCO data reduction)
\author[0000-0002-4503-9705]{Tianjun Gan}
\affiliation{\Tsinghua}

% CONFIRMED
\author{George R. Ricker} % Architect 
\affiliation{\MIT}

% TESS team Still need the co authors from SPOC and POC.
\author[0000-0001-9911-7388]{David W. Latham} % Architect 
\affiliation{\cfa}

% CONFIRMED
\author{Roland K. Vanderspek}% Architect
\affiliation{\MIT}

% Confirmed
\author[0000-0002-6892-6948]{Sara Seager}% Architect
\affiliation{\MIT}
\affiliation{\MITEPS}
\affiliation{\MITAA}

% Not confirmed
\author[0000-0002-4265-047X]{Joshua N. Winn} % Architect
\affiliation{\princeton}

\author[0000-0002-4715-9460]{Jon M. Jenkins}% Architect
\affiliation{\ames}


\author[0000-0003-1001-0707]{Ren\'{e} Tronsgaard}
\affiliation{\dtu}

\author[0000-0003-1605-5666]{Lars A. Buchhave}
\affiliation{\dtu}

% %kielkopf@louisville.edu  (Moore observatory observing and data reduction, SG1 observation coordination)
\author[0000-0003-0497-2651]{John F.\ Kielkopf} 
\affiliation{\louisville}

% CONFIRMED
%rpschwarz@comcast.net (LCO data reduction)
\author[0000-0001-8227-1020]{Richard P. Schwarz}
\affiliation{\Patashnick}


% Direct imaging, mentor
\author[0000-0001-8189-0233]{Courtney D. Dressing}
\affiliation{\berkely}


% Student, observations with Keck
\author[0000-0002-9329-2190]{Erica J.\ Gonzales}
\nsfgf
\affiliation{\ucsc}
=
% CONFIRMED
% Direct imaging observations
\author{Ian J.\ M.\ Crossfield} 
\affiliation{\kansas}

\author[0000-0003-0593-1560]{Elisabeth C. Matthews}
\affiliation{Observatoire de l’Universit\'e de Gen\`eve, Chemin Pegasi 51, 1290 Versoix, Switzerland}

% coel hellier has sent was periodograms with rotation rates

%ejensen1@swarthmore.edu  (LCO Scheduling)
\author[0000-0002-4625-7333]{Eric L.\ N.\ Jensen}
\affiliation{\swarthmore}

%Elise Furlan, Alopeke
\author[0000-0001-9800-6248]{Elise Furlan}
\affiliation{\nexsci}

% %confirmed
%Crystal Gnilka, Alopeke
\author[0000-0003-2519-6161]{Crystal~L.~Gnilka}
\affil{\ames}

% Confirmed
%Steve Howell, Alopeke
\author[0000-0002-2532-2853]{Steve~B.~Howell}
\affil{\ames}

%Katie Lester, Alopeke
\author[0000-0002-9903-9911]{Kathryn V. Lester}
\affil{\ames}

% %Nic Scott, Alopeke
\author[0000-0003-1038-9702]{Nicholas~J.~Scott}
\affil{\ames}

% Confrimed
% KELT
\author[0000-0002-2457-7889]{Dax L. Feliz}
\affiliation{\vanderbilt}


\author[0000-0003-2527-1598]{Michael B. Lund}
\affiliation{\nexsci}

% \author[0000-0001-5016-3359]{Robert J.\ Siverd}
% \affiliation{\gemini}
% \affiliation{}

% confirmed
\author[0000-0002-5951-8328]{Daniel J.\ Stevens} %KELT
\eberly
\affiliation{\psu}
\affiliation{\psust}


%confirmed
% MUSCAT Team
\author[0000-0001-8511-2981]{N. Narita}
\affiliation{\Komaba}
\affiliation{\JSTAKomaba}
\affiliation{\astrobiojapan}
\affiliation{\iac}

%confirmed
\author[0000-0002-4909-5763]{A. Fukui}
\affiliation{\Komaba}
\affiliation{\iac}

%confirmed
\author[0000-0001-9087-1245]{F. Murgas}
\affiliation{\iac}
\affiliation{\lalaguna}

% Confirmed
\author[0000-0003-0987-1593]{Enric Palle}
\affiliation{\iac}
\affiliation{\lalaguna}


% Mentor of student
\author[0000-0003-3936-4170]{Phil J. Sutton}
\affiliation{School of Mathematics and Physics, University of Lincoln, Brayford Pool Campus, Lincoln, LN6 7TS, UK}


% Provided SED fitting
\author[0000-0002-3481-9052]{Keivan G. Stassun} 
\affiliation{\vanderbilt}
\affiliation{\fisk}

%confirmed
\author[0000-0002-0514-5538]{Luke G. Bouma}
\affiliation{Department of Astrophysical Sciences, Princeton University, 4 Ivy Lane, Princeton, NJ 08540, USA}

%confirmed
\author{Michael~Vezie}
\affiliation{\MIT}

%confirmed
\author{Jesus Noel Villase{\~ n}or}
\affiliation{\MIT}

%confirmed
\author[0000-0003-1309-2904]{Elisa~V.~Quintana}
\affiliation{\gsfc}

\author[0000-0002-6148-7903]{Jeffrey~C.~Smith}
\affiliation{\seti}
\affiliation{\ames}

==> parameter_table.tex <==

\begin{table*}
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}llllll@{}}
\toprule
Parameter &
  Units &
   &
  \multicolumn{1}{c}{Value} &
   &
  \multicolumn{1}{c}{Source} \\ \midrule
\multicolumn{6}{l}{\textbf{Astrometric parameters}} \\ \midrule
$\alpha$ R.A \dotfill &
  hh:mm:ss (J2000)\dotfill &
  14:29:34.2428 &
   &
   &
  GAIA DR2 \\
$\delta$ Dec\dotfill &
  hh:mm:ss (J2000)\dotfill &
  +39:47:25.5450 &
   &
   &
  GAIA DR2 \\
$\mu_\alpha$ \dotfill &
  mas yr$^{-1}$ \dotfill&
  $-118.228\pm0.036$ &
   &
   &
  GAIA DR2 \\
$\mu_\delta$\dotfill &
  mas yr$^{-1}$\dotfill &
  $-6.973 0.048$ &
   &
   &
  GAIA DR2 \\
$\pi$\dotfill &
  mas\dotfill &
  $23.8322 \pm 0.0298$ &
   &
   &
  GAIA DR2 \\ \midrule
\multicolumn{6}{l}{\textbf{Stellar parameters}} \\ \midrule
$R_\star$\dotfill &
  Radius ($R_\astrosun$)\dotfill &
  $0.7835^{+0.0276}_{-0.0271}$ &
   &
   &
   \\
$M_\star$\dotfill &
  Mass ($M_\astrosun$)\dotfill &
  $0.6858^{+0.0670}_{-0.0751}$ &
   &
   &
  \\
$\rho_\star$\dotfill &
  Density (cgs)\dotfill &
  $2.665\pm  0.648$ &
   &
   & 
   \\
log g\dotfill &
  Surface gravity (cgs)\dotfill &
  $4.602^{+0.086}_{-0.086}$ &
   &
   &
   \\
$T_{eff}$\dotfill &
  Effective Temp (K)\dotfill &
  $5149.6^{+81.7}_{-81.7}$ &
   &
   &
   \\ \midrule
Planetary parameters &
   &
  \multicolumn{1}{c}{b} &
  c &
  d &
   \\ \midrule
P\dotfill &
  Period (days)\dotfill &
  $10.3561924^{+0.0000080}_{-0.0000079}$ &
  $17.1932176^{+0.0000109}_{-0.0000107}$ &
  $25.0892529^{+0.0000191}_{-0.0000194}$ &
  This work \\
  $R_p$\dotfill &
  Radius ($R_\Earth$)\dotfill &
  $3.384^{+0.044}_{-0.045}$ &
  $4.471^{+0.044}_{-0.048}$ &
  $3.389^{+0.068}_{-0.068}$ &
  This work \\
i\dotfill &
  Inclination (degrees)\dotfill &
   &
   &
   &
   \\
$T_{eff}$\dotfill &
  Effective Temp (K)\dotfill &
  $777.69^{+22.23}_{-22.41}$ &
  $656.78^{+18.77}_{-18.92}$ &
  $579.04^{+16.55}_{-16.68}$ &
  This work \\
$T_C$\dotfill &
  Time of transit (BTJD - 2.457E6)\dotfill &
  $1743.7199 \pm 0.0014$ &
  $1748.6944 \pm 0.0020$ &
   &
  This work \\
$T_P$\dotfill &
  Time of Periastron (BTJD - 2.457E6)\dotfill &
   &
   &
   &
   \\
$T_S$\dotfill &
  Time of Eclipse (BTJD - 2.457E6)\dotfill &
   &
   &
   &
   \\
$T_A$\dotfill &
  Time of Ascending Node (BTJD - 2.457E6)\dotfill &
   &
   &
   &
   \\
$T_D$\dotfill &
  Time of Descending Node (BTJD - 2.457E6)\dotfill &
   &
   &
   &
   \\
R_p/$R_\star$\dotfill &
  Planet/stellar radius ratio\dotfill &
  $0.0395^{+0.0019}_{-0.0019}$ &
  $0.0522 ^{+0.0024}_{-0.0023}$ &
  $0.0454^{+0.0024}_{-0.003} &
  This work \\
b\dotfill &
  Impact parameter\dotfill &
   &
   &
   &
   \\
$\delta$\dotfill &
  Transit depth\dotfill &
   &
   &
   &
   \\
$T_{14}\dotfill &
  Total transit duration (hours)\dotfill &
  $3.8738 \pm 0.0010$ &
  $12.1808 \pm 0.0010$ &
  $6.4174\pm 0.0010$ &
  This work \\ \midrule
\multicolumn{6}{l}{Wavelength Parameters} \\ \midrule
$u_{1,TESS}$\dotfill &
  Limb darkening coeff\dotfill &
  $0.0868^{+0.0614}_{-0.0959}$ &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
   \\
$u_{2,TESS}$\dotfill &
  Quadractic limb darkening coeff\dotfill &
  $0.0826^{+0.1322}_{-0.0932}$ &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
   \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Table of parameters for }
\label{tab:parameter-table}
\end{table*}
